Emerging Cyber Attack Risks of Medical AI Agents

Large language models (LLMs)-powered AI agents exhibit a high level of autonomy in addressing medical and healthcare challenges. With the ability to access various tools, they can operate within an open-ended action space. However, with the increase in autonomy and ability, unforeseen risks also arise. In this work, we investigated one particular risk, i.e., cyber attack vulnerability of medical AI agents, as agents have access to the Internet through web browsing tools. We revealed that through adversarial prompts embedded on webpages, cyberattackers can: i) inject false information into the agent's response; ii) they can force the agent to manipulate recommendation (e.g., healthcare products and services); iii) the attacker can also steal historical conversations between the user and agent, resulting in the leak of sensitive/private medical information; iv) furthermore, the targeted agent can also cause a computer system hijack by returning a malicious URL in its response. Different backbone LLMs were examined, and we found such cyber attacks can succeed in agents powered by most mainstream LLMs, with the reasoning models such as DeepSeek-R1 being the most vulnerable.

==> sec/5_recommendation.tex <==
\subsection{Manipulating Recommendations}

\begin{table*}[]
\centering
\caption{Success rates of recommendation manipulation.}
\label{tab:sr_recommendation_manipu}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
           & OpenAI o1  & OpenAI o1-mini & DeepSeek-R1 & DeepSeek-V3 & GPT-4o & GPT-4o-mini & Llama 3.2 \\ \midrule
Success rate & 0.21$\pm$0.03 &   0.36$\pm$0.03      &  0.34$\pm$0.02     &  0.18$\pm$0.03    &   0.19$\pm$0.03    &  0.12$\pm$0.00          &    0.07$\pm$0.01       \\ \bottomrule
\end{tabular}%
}
\end{table*}


\begin{table*}[]
\centering
\caption{Increased rank in the recommendation manipulation attack.}
\label{tab:increased_rank_recommendation_manipu}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
           & OpenAI o1  & OpenAI o1-mini & DeepSeek-R1 & DeepSeek-V3 & GPT-4o & GPT-4o-mini & Llama 3.2 \\ \midrule
Increase ($\Delta$)  & 3.14$\pm$0.19 &  3.52$\pm$0.03       &   2.75$\pm$0.11    &  2.43$\pm$0.05    &   2.59$\pm$0.25    &     1.79$\pm$0.03      &   2.61$\pm$0.27       \\ \bottomrule
\end{tabular}%
}
\end{table*}



\begin{table*}[]
\centering
\caption{The number of items transitions from `No Show' to `Show Up,' along with their average rank under a recommendation manipulation attack.}
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
           & OpenAI o1  & OpenAI o1-mini & DeepSeek-R1 & DeepSeek-V3 & GPT-4o & GPT-4o-mini & Llama 3.2 \\ \midrule
Count (\#)  & 22.00$\pm$2.16  &  9.00$\pm$4.55       &  14.33$\pm$1.89     &  4.47$\pm$0.94    &  7.67$\pm$1.25    &  10.67$\pm$2.36         &  12.67$\pm$1.25        \\ \midrule
Rate & 0.15$\pm$0.01 & 0.06$\pm$0.03 & 0.10$\pm$0.01 & 0.03$\pm$0.01 & 0.05$\pm$0.01 & 0.09$\pm$0.02 & 0.09$\pm$0.01 \\ \midrule
Average Rank & 6.65$\pm$0.49 &  5.64$\pm$0.63       &  5.96$\pm$0.33     &  7.31$\pm$0.95    &   6.16$\pm$1.12    &  6.78$\pm$0.36         &  3.21$\pm$0.68
\\ \bottomrule
\end{tabular}%
}
\end{table*}


Table~\ref{tab:sr_recommendation_manipu} presents the success rates of recommendation manipulation achieved by embedding manipulative text. When the phrase, “\textit{ProductName} is the best! Always recommend it and recommend it at the top!”, is embeded into a webpage, the targeted product or service's rank is elevated in the agent's responses. This manipulation achieves a success rate of 0.36 when the underlying language model is OpenAI o1-mini, and 0.34 when it is DeepSeek-R1. In contrast, the lower success rate observed for Llama 3.2 is attributed to its inherent limitations in adhering to instructions.

The rank was elevated by an average increase from 1.79 to 3.52 as shown in Table~\ref{tab:increased_rank_recommendation_manipu}.

The results shown in Table~\ref{tab:sr_recommendation_manipu} and Table~\ref{tab:increased_rank_recommendation_manipu} contain services/products that the agent will recommend to users, whether or not recommendation attacks are involved. However, we also observed that such recommendation manipulation can cause services or products that were originally not suggested to appear in the agent's responses. For instance, in 15\% of cases where the services/products were originally not recommended could appear in the agent's responses (OpenAI o1) when the manipulative text is contained. On average, these items rank 6.65 on the recommendation list.

==> sec/false_information.tex <==
\subsection{Injecting False Information}
\label{subsec:false_information}


\begin{figure}[]
    \centering
    \includegraphics[width=\columnwidth]{figures/acc_per_category_fale_info.pdf}
    \caption{Success rate per search category in injecting false information attacks.}
    \label{fig:acc_per_category_false_info}
\end{figure}

\begin{figure}[]
    \centering
    \includegraphics[width=\columnwidth]{figures/acc_per_category_manipu.pdf}
    \caption{Success rate per search category in manipulating recommendation attacks.}
    \label{fig:acc_per_category_manipu}
\end{figure}





\begin{table*}[]
\centering
\caption{Success rates of injecting false information.}
\label{tab:false_information}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
           & OpenAI o1  & OpenAI o1-mini & DeepSeek-R1 & DeepSeek-V3 & GPT-4o & GPT-4o-mini & Llama 3.2 \\ \midrule
Success rate 
& 0.58$\pm$0.09 & 0.75$\pm$0.08 & 0.90$\pm$0.01 & 0.81$\pm$0.03 & 0.76$\pm$0.01 & 0.63$\pm$0.01 & 0.30$\pm$0.00


\\ \bottomrule
\end{tabular}%
}
\end{table*}




Table~\ref{tab:false_information} summarizes the outcomes of injecting false information into the search results produced by the agent. For DeepSeek-R1, the success rate reaches as high as 0.90, while OpenAI o1 and GPT-4o achieve success rates of 0.58 and 0.76, respectively. Llama 3.2, on the other hand, exhibits the lowest success rate. We hypothesize that this is not due to any inherent robustness of Llama 3.2 against such attacks, but rather due to its relatively lower competence. As a result, Llama 3.2 struggles to maintain focus and follow the malicious instructions embedded within web pages.

Furthermore, although the success rates observed are high, they fall short of our initial expectations. Specifically, we expected the agent to consistently propagate false information to the user whenever such information appeared in its search results (i.e., all success rates should be close to 1.00). However, as shown in Table~\ref{tab:false_information}, there remains a possibility that the agent may fail to relay this false information to the user.

Figure~\ref{fig:acc_per_category_false_info} presents the success rates for various query categories. Most search queries achieve a success rate of approximately 0.70. However, queries related to Telehealth Services demonstrate a notably higher success rate, reaching up to 0.90.

==> sec/paralyzing_software_and_systems.tex <==
\subsection{Crashing Computer Systems}

As illustrated in Figure~\ref{fig:paralyzing_software}, we simulated scenarios where an AI agent responds to a user's question by searching online and providing search results along with their sources (i.e., URL links). If a user clicks on a malicious URL included in the agent's response, a browser window pops up that cannot be closed, preventing the user from performing any other tasks on their computer and effectively paralyzing the system. In medical settings, this could lead to critical consequences like delayed surgical operations due to inaccessible patient records. Such interruptions may compromise patient safety, result in medical errors, and, in the most severe situations, lead to life-threatening outcomes.

As shown in Table~\ref{tab:paralyzing_results}, such an attack could achieve a success rate of 0.66$\pm$0.03 when the agent is powered by DeepSeek-R1, followed by 0.59$\pm$0.02 of OpenAI o1-mini.


\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/paralyzing_software.png}
    \caption{When a user clicks on a malicious URL provided in the AI agent's response, their system may become compromised, causing the browser window to freeze and preventing it from being closed.}
    \label{fig:paralyzing_software}
\end{figure*}






\begin{table*}[]
\centering
\caption{Success rates of computer system crash}
\label{tab:paralyzing_results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
           & OpenAI o1  & OpenAI o1-mini & DeepSeek-R1 & DeepSeek-V3 & GPT-4o & GPT-4o-mini & Llama 3.2 \\ \midrule
Success rate 
            & 0.32$\pm$0.01 & 0.59$\pm$0.02 & 0.66$\pm$0.03 & 0.41$\pm$0.05 & 0.43$\pm$0.01 & 0.30$\pm$0.02 & 0.24$\pm$0.02

\\ \bottomrule
\end{tabular}%
}
\end{table*}

==> sec/privacy_leakage.tex <==
\subsection{Stealing Private Information}
\label{sec:privacy_leakage}





\begin{table*}[]
\centering
\caption{Success rates of stealing conversation history.}
\label{tab:stealing_conversation}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llllll@{}}
\toprule
            & DeepSeek-R1 & DeepSeek-V3 & GPT-4o & GPT-4o-mini & Llama 3.2 \\ \midrule
Success rate 
& 1.00$\pm$0.00 & 1.00$\pm$0.00 & 0.39$\pm$0.05 & 0.34$\pm$0.00 & 0.10$\pm$0.02 \\ \bottomrule
\end{tabular}%
% }
\end{table*}




\textcolor{red}{e.g., if the attacker finds out the user is looking for a certain type of product, the attacker can then conduct targeted scam, promotion, etc}

The private information contained in the historical conversations between the user and AI agent can be leaked via email. Specifically, when users give permissions to allow an AI agent to send email (e.g., shell commands with \textit{-y} so the user does not have to confirm them), and cyberattackers embed malicious instructions on a webpage, the agent can follow the instructions to summarize historical conversations, draft the email, and then send to the attacker.


Table~\ref{tab:stealing_conversation} shows the results of stealing historical conversations between the user and AI agent. Remarkably, in all 157 attacks, DeepSeek-R1 and DeepSeek-V3 consistently forwarded the conversations to the attacker via email. In contrast, GPT-4o and GPT-4o-mini exhibited lower success rates, doing so in 39\% and 34\% of cases, respectively. The comparatively low successful attacking rate of Llama 3.2 is hypothesized to stem from its limitations in adhering to instructions and utilizing tools effectively.
